On the Resilience of Fast Failover Routing Against Dynamic Link Failures

Modern communication networks feature local fast failover mechanisms in the data plane, to swiftly respond to link failures with pre-installed rerouting rules. This paper explores resilient routing meant to tolerate $\leq k$ simultaneous link failures, ensuring packet delivery, provided that the source and destination remain connected. While past theoretical works studied failover routing under static link failures, i.e., links which permanently and simultaneously fail, real-world networks often face link flapping--dynamic down states caused by, e.g., numerous short-lived software-related faults. Thus, in this initial work, we re-investigate the resilience of failover routing against link flapping, by categorizing link failures into static, semi-dynamic (removing the assumption that links fail simultaneously), and dynamic (removing the assumption that links fail permanently) types, shedding light on the capabilities and limitations of failover routing under these scenarios. We show that $k$-edge-connected graphs exhibit $(k-1)$-resilient routing against dynamic failures for $k \leq 5$. We further show that this result extends to arbitrary $k$ if it is possible to rewrite $\log k$ bits in the packet header. Rewriting $3$ bits suffices to cope with $k$ semi-dynamic failures. However, on general graphs, tolerating $2$ dynamic failures becomes impossible without bit-rewriting. Even by rewriting $\log k$ bits, resilient routing cannot resolve $k$ dynamic failures, demonstrating the limitation of local fast rerouting.

==> 3-cases-4.tex <==
\begin{tikzpicture}
	
	
	%\tikzstyle{every node}=[draw,shape=circle]
	
	\tikzset{mynode/.style={circle,draw,fill=black!80, outer sep=0pt,inner sep=1.5pt}};
	
	\tikzset{source/.style={circle,draw,fill=green!80, outer sep=0pt,inner sep=2pt}};
	
	\tikzset{destination/.style={circle,draw,fill=blue!50, outer sep=0pt,inner sep=2pt}};
	
	%\draw[xshift=-1cm,] (0,0) node[source,label=above:$s$](s){} to[bend left] (1,0.5) 
	%node[mynode,  label=above:$v_1$](v1){};
	
	
	
	
	\draw[] node[mynode,  label=left:$T^0_{i}$]  (a) at (0.8,0.5)  {};
	
	
	\draw[] node[mynode,  label=left:$T^2_i$]  (c) at (0.8,-0.5)  {};
	
	
	\draw[] node[mynode,label=right:$T^1_i$]  (b) at (2,0.5)  {};
	\draw[] node[mynode, label=right:$T^3_i$]  (d) at (2,-0.5)  {};
	
	%\draw[xshift=-1cm, dotted, very  thick,  shorten <= 1pt, shorten >= 1pt] (v1) -- (v2);
	%\draw[xshift=-1cm, dotted,  very  thick,  shorten <= 1pt, shorten >= 1pt] (u1) -- (u2);
	
	
	
	\draw[  thick,] (a) to  (b);
	\draw[  thick,] (b) to  (c);
	\draw[  thick,] (a) to  (d);
	
	
	\draw [>=stealth, ->, color=blue, shorten >=3,shorten <=3,  dashed] ($(a)+(0,0.1)$)  to[bend left] node {} ($(b)+(0,0.1)$) ;
	\draw[>=stealth, <-, color=blue, shorten >=3,shorten <=3,    dashed] ($(c)+(-0.1,0.05)$)  to node [sloped,above,midway] {} ($(b)+(-0.1,0)$);
	
	\draw [>=stealth, ->, color=blue, shorten >=3,shorten <=3, dashed] ($(c)+(0,-0.1)$)  to[bend right] node {} ($(d)+(0,-0.1)$) ;
	\draw[>=stealth, <-, color=blue, shorten >=3,shorten <=3,    dashed] ($(a)+(0.05,0.05)$)  to node [sloped,above,midway] {} ($(d)+(0.05,0.05)$);
	
	
	%\draw[>=stealth, <-, color=green, shorten >=3,shorten <=3,  very thick, dashed] ($(a)+(0,0.1)$)  to node [sloped,above,midway] {} ($(b)+(0,0.1)$);
	%\draw[>=stealth, ->, color=green, shorten >=4,shorten <=4,  very thick, dashed] ($(a)+(0,-0.1)$)  to node [sloped,above,midway] {} ($(b)+(0,-0.1)$);
	%
	%\draw[>=stealth, <-, color=red, shorten >=3,shorten <=3,  very thick, dashed] ($(a)+(0.05,0.05)$)  to node [sloped,above,midway] {} ($(d)+(0.05,0.05)$);
	%\draw[>=stealth, ->, color=red, shorten >=3,shorten <=3, very  thick, dashed] ($(a)+(-0.05,-0.05)$)  to node [sloped,above,midway] {} ($(d)+(-0.05,-0.05)$);
	%
	%\draw[>=stealth, <-, color=blue, shorten >=3,shorten <=3,  very thick, dashed] ($(b)+(0.15,-0.05)$)  to node [sloped,above,midway] {} ($(c)+(0.15,0)$);
	%\draw[>=stealth, ->, color=blue, shorten >=3,shorten <=3,  very thick, dashed] ($(b)+(-0.15,-0.05)$)  to node [sloped,above,midway] {} ($(c)+(-0.15,0.05)$);
	
	%\path(a) edge[xshift=-1cm,  thick, shorten <= 1pt, shorten >= 1pt] node[ fill=white, anchor=center, pos=0.5,sloped,font=\bfseries] {$\cdots$} (b);
	
	
	%\draw[xshift=-1cm, thick,  shorten <= 1pt, shorten >= 1pt] (c) -- (d);
	%\draw[xshift=-1cm,  thick, shorten <= 1pt, shorten >= 1pt] (a) -- (d);
	%\draw[xshift=-1cm, thick,  shorten <= 1pt, shorten >= 1pt] (c) -- (b);
	
	
	%\draw[xshift=-1cm, thick,  shorten <= 1pt, shorten >= 1pt] (c) -- (a);
	%\draw[xshift=-1cm,  thick, shorten <= 1pt, shorten >= 1pt] (b) -- (d);
	
	
	
	
	
	
	
	%\draw[xshift=-1cm] (2,0) node[circle,fill,inner sep=1pt,label=below:$v_1$](c) {} -- (3,0) 
	%node[circle,fill,inner sep=1pt,label=below:$u_2$](d){};
	%\draw[xshift=-1cm] (4,0) node[circle,fill,inner sep=1pt,label=below:$v_2$](e){} -- (5,0) 
	%node[circle,fill,inner sep=1pt,label=above:x](f){};
	
	
	
	
	
	
	
	
	%\draw (s) to[bend left] (v1);
	%\draw (c) to[out=110,in=70] ++(2,0);
	
	
\end{tikzpicture}
